Learn by Guessing: Multi-Step Pseudo-Label Refinement for Person Re-Identification

Unsupervised Domain Adaptation (UDA) methods for person Re-Identification (Re-ID) rely on target domain samples to model the marginal distribution of the data. To deal with the lack of target domain labels, UDA methods leverage information from labeled source samples and unlabeled target samples. A promising approach relies on the use of unsupervised learning as part of the pipeline, such as clustering methods. The quality of the clusters clearly plays a major role in methods performance, but this point has been overlooked. In this work, we propose a multi-step pseudo-label refinement method to select the best possible clusters and keep improving them so that these clusters become closer to the class divisions without knowledge of the class labels. Our refinement method includes a cluster selection strategy and a camera-based normalization method which reduces the within-domain variations caused by the use of multiple cameras in person Re-ID. This allows our method to reach state-of-the-art UDA results on DukeMTMC-Market1501 (source-target). We surpass state-of-the-art for UDA Re-ID by 3.4% on Market1501-DukeMTMC datasets, which is a more challenging adaptation setup because the target domain (DukeMTMC) has eight distinct cameras. Furthermore, the camera-based normalization method causes a significant reduction in the number of iterations required for training convergence.

==> Sections/Anotacoes.tex <==
*Introdução - Linha 66:*

_% (\eg dense multi-camera clusters). ==> NAO ENTENDI ISSO EM PARENTESES, ESSE TERMO EH BEM CONHECIDO NA COMUNIDADE OU VOCE INVENTOU?_

*Resposta:* Eu inventei, queria dizer clusters densos (com muitos samples) e multi-camera (com samples de diferentes cameras)

======================================================================================================

*Introdução - Linha 74:*

_% TA CERTO ISSO, "DUAL DATASET"?_

*Resposta:* Não sei, eu inventei também

======================================================================================================

*Introdução - Linha 82:*

_NAO TEM MAIS CONTRIBUICOES NA METODOLOGIA? VOCE SEMPRE FALA DE COISAS QUE VOCE PROPOS E QUE NUNCA HAVIA VISTO EM ARTIGOS PUBLICADOS..._

*Resposta:* O que eu digo que nunca vi é a seleção de clusters, mas ela ta inclusa no método que refina os clusters, por isso não indiquei explicitamente nas contribuições

======================================================================================================

*Related Works - Linha 36:*

_% CHECK IF IT REALLY MAKES SENSE TO REPLACE CAMERA BY DATASET HERE!_

*Reposta:* Acredito que não faz sentido, pois ele aplica isso já nas images do target domain e ele deseja simular as outras cameras do target domain. Então acho que camera fica melhor (ja fiz a mudança no overleaf

======================================================================================================

*Related Works - Linha 52:*

_% O QUE SAO "INTERESTING REGIONS"???_

*Reposta:* Seriam as regiões mais densas, onde os pontos estão concentrados. Acho que a ideia que quis passar era de melhorar o modelo para que os outliers entrem nos clusters e não sejam mais outliers.

======================================================================================================

*Methodology - Linha 10:*

_% DO WE REALLY INTRODUCE? IT WAS "TALK ABOUT" BEFORE, BUT THAT'S TOO INFORMAL._

*Reposta:* Não sei se introduce é a melhor palavra pq não fomos nós que propomos, a fonte é citada em 3.2

======================================================================================================

*Methodology - Linha 32:*

_% NAO SEI SE ENTENDO BEM O QUE VOCE QUIS DIZER COM A FRASE ACIMA..._

*Reposta:* Os blocos residuais facilitam que a rede aprenda um bypass, então eu quis argumentar que isso facilita levar informações de camadas mais razas para camadas mais fundas. E como reid precisa de multiplas camadas semanticas, a informação importante para a feature final estará espalhada nessas camadas.

======================================================================================================

*Methodology - Linha 72:*

_% AFINAL, COMO EH QUE VOCE GARANTE QUE NOVOS PSEUDO-LABELS SAO MAIS_
_% PROXIMOS DO ROTULO REAL?_
_% COMO VOCE SABE SE O DADO EH RELIABLY?_
_% ME DEU A IMPRESSAO DE QUE ESSE SEGUNDO PARAGRAFO NA VERDADE SE TRATA_
_% DO QUE A SECAO 3.4 FAZ._

*Reposta:* Acho que eu concordo, realmente é a seção 3.4 que "garante" essa melhoria continua

======================================================================================================

*Methodology - Linha 145:*

_% HOW DID YOU DETERMINE \epsilon?_

*Reposta:* Foi tentativa e erro tentando equilibrar o número de clusters e o a quantidade de outliers 

======================================================================================================

*Methodology - Linha 147:*

_% A PALAVRA INTELLIGENT EH PERIGOSA... ESSE METODO NAO EH MUITO INTELIGENTE..._

*Reposta:* Concordo, será que é melhor deixar só Cluster Selection

======================================================================================================

*Methodology - Linha 168:*

_% I'VE EDITED THE PARAGRAPH BELOW, PLEASE SEE IF IT STILL MAKES SENSE:_

*Reposta:* Fiz uma pequena alteração, não tinha entendido o termo "propose to use guarantee that"

======================================================================================================

*Methodology - Linha 174:*

_% WAS THIS DONE FOR K-MEANS AS WELL?_

*Reposta:* Sim

======================================================================================================

*Methodology - Linha 189:*

_% WILL WE REALLY CALL IT "INTELLIGENT"?_

*Reposta:* Não me importo de tirar o intelligent, mantive apenas por coerência

======================================================================================================

*Methodology - Linha 197:*

_% O QUE VOCE QUER DIZER COM CHANGE THE MODEL? RETREINAR?_

*Reposta:* Mudar a arquitetura, sem precisar trocar as camadas de batch normalization por camera batch normalization (inseri a palavra architecture no final do paragrafo)

======================================================================================================

*Methodology - Linha 213:*

_% MEDIA E DESVIO PADRAO SAO VETORES OU ESCALARES, I.E., VOCE CALCULA POR FEATURE OU GLOBALMENTE?_

*Reposta:* São vetores. Calculo os vetores para cada camera e depois aplico nas features daquela camera

++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
					                    NOVAS RESPOSTAS
++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++
++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++++

======================================================================================================

*Methodology - Linhas 235 e 252:*

_% HOW DID YOU COME UP WITH THE WEIGHT 0.005. IS THIS USED IN OTHER PAPERS?_
_% TELL WHERE THIS RATE SCHEDULER CAME FROM AND HOW YOU DECIDED THESE PARAMETERS._

*Reposta:* Ambos vieram do paper  Bag of tricks and a strong baseline for deep personre-identification  (\cite{Luo_2019_CVPR_Workshops})

======================================================================================================

*Methodology - Linha 271:*

_% NAO ENTENDI ESSE TRECHO ACIMA:
% "learn a good enough $\p$ to control the $\mathcal{L}_{\textit{ID}}$." 
% A IDEIA EH MANTER A CROSS ENTROPY SUB CONTROLE?
% EU ENTENDI QUE ESSE FINE TUNING SEPARA CORPO DE CABECA (E ESCREVI DE ACORDO),
% (O QUE EH UMA TECNICA PADRAO EM FINE TUNING). ENTENDI CORRETAMENTE?_

*Reposta:* Isso, entendeu corretamente sim! O que eu quis dizer ali é que a cada passo do progressive learning clusterização é refeita, então as vezes a imagem que tinha o ID 10 passa a ter o ID 232 na próxima etapa, ai o vetor p não faz sentido mais e a cross entropy vai la pra cima. Então eu congelo tudo, menos a fully connected que leva as features pra p até a cross entropy voltar pra um patamar mais normal, pra nao correr o risco do alto gradiente de erro gerado por ela atrapalhar o aprendizado prévio da triplet loss.

======================================================================================================

*Methodology - Linha 279:*

_% COMO VOCE CALCULA MEAN AP? VOCE USA ROTULOS DO TARGET SET??? _

*Reposta:* Sim, pra calcular o Mean AP eu uso os rotulos de test do target set. Eu acho muito estranho isso fazer parte de um passo de adaptação de domínio, mas acredito que todo mundo faça. Inclusive, no paper Hierarchical Clustering With Hard-Batch Triplet Loss for Person Re-Identification (\cite{HCT}) eles falam explicitamente que fazem isso e eles tambem usam progressive learning

======================================================================================================

*Introdução - Linha 57:*

_% SOFT OU SOFT-LIKE? O QUE EH SOFT-LIKE?_

*Resposta:* Eu inventei soft-like, é soft mesmo

